Hunting for exoplanets via magnetic star-planet interactions: geometrical considerations for radio emission

Recent low-frequency radio observations suggest that some nearby M dwarfs could be interacting magnetically with undetected close-in planets, powering the emission via the electron cyclotron maser (ECM) instability. Confirmation of such a scenario could reveal the presence of close-in planets around M dwarfs, which are typically difficult to detect via other methods. ECM emission is beamed, and is generally only visible for brief windows depending on the underlying system geometry. Due to this, detection may be favoured at certain orbital phases, or from systems with specific geometric configurations. In this work, we develop a geometric model to explore these two ideas. Our model produces the visibility of the induced emission as a function of time, based on a set of key parameters that characterise magnetic star-planet interactions. Utilising our model, we find that the orbital phases where emission appears are highly dependent on the underlying parameters, and does not generally appear at the quadrature points in the orbit as is seen for the Jupiter-Io interaction. Then using non-informative priors on the system geometry, we show that untargeted radio surveys are biased towards detecting emission from systems with planets in near face-on orbits. While transiting exoplanets are still likely to be detectable, they are less likely to be seen than those in near face-on orbits. Our forward model serves to be a powerful tool for both interpreting and appropriately scheduling radio observations of exoplanetary systems, as well as inverting the system geometry from observations.

==> complog <==
This is pdfTeX, Version 3.141592653-2.6-1.40.25 (TeX Live 2023) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2022-11-01> patch level 1
L3 programming layer <2023-02-22> (./mnras.cls
Document Class: mnras 2015/05/22\ v3.0\ LaTeX2e MNRAS document class
MNRAS document style v3.0, released 2015/05/22
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.
sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
 (/usr/local/texlive/2023basic/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/gettitlestring/gettitlestr
ing.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/kvoptions/kvoptions.sty)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty)
) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/atbegshi-ltx.sty)

Package hyperref Warning: Option `pdfpagelabels' is turned off
(hyperref)                because \thepage is undefined.

) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/rerunfilecheck/rerunfilechec
k.sty (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/atveryend-ltx.sty
)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/uniquecounter/uniquecounte
r.sty))) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/natbib/natbib.sty))
 (/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/newtxtext.sty
`newtxtext' v1.71, 2022/02/28 Text macros taking advantage of TeXGyre Termes an
d its extensions (msharpe)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/textcomp.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/carlisle/scalefnt.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kastrup/binhex.tex)
ntx@otftextfalse
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/fontaxes/fontaxes.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.71, 2022/01/16 Math macros based originally on txfonts (msharpe)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifxetex.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifluatex.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kastrup/binhex.tex)
amsthm NOT loaded
) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fontenc.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1minntx.fd))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/ae.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fontenc.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/aecompl.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/mathcolor.ltx))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1ntxtlf.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/l3backend/l3backend-pdftex.d
ef)
No file main.aux.
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/omlntxmi.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/local/texlive/2023basic/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.s
ty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg
)) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/ot1minntx.fd)

LaTeX Font Warning: Font shape `OML/cmm/b/it' in size <10.5> not available
(Font)              size <10.95> substituted on input line 34.

(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/ueur.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxsyc.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1ntxsups.fd)

LaTeX Font Warning: Font shape `OML/cmm/b/it' in size <5.5> not available
(Font)              size <5> substituted on input line 34.

(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/t1aett.fd)

Package natbib Warning: Citation `nicholson19' on page 1 undefined on input lin
e 54.


Package natbib Warning: Citation `burn21' on page 1 undefined on input line 54.



Package natbib Warning: Citation `winters19' on page 1 undefined on input line 
54.


Package natbib Warning: Citation `burn21' on page 1 undefined on input line 54.



Package natbib Warning: Citation `schlecker22' on page 1 undefined on input lin
e 54.


Package natbib Warning: Citation `zarka07' on page 1 undefined on input line 56
.


Package natbib Warning: Citation `saur13' on page 1 undefined on input line 56.



Package natbib Warning: Citation `alfven42' on page 1 undefined on input line 5
6.


Package natbib Warning: Citation `neubauer80' on page 1 undefined on input line
 56.


Package natbib Warning: Citation `dulk85' on page 1 undefined on input line 56.



Package natbib Warning: Citation `treumann06' on page 1 undefined on input line
 56.


Package natbib Warning: Citation `vidotto14' on page 1 undefined on input line 
64.


LaTeX Warning: Reference `firstpage' on page 1 undefined on input line 65.


LaTeX Warning: Reference `lastpage' on page 1 undefined on input line 65.

(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/ts1ntxtlf.fd) [1{/usr/
local/texlive/2023basic/texmf-var/fonts/map/pdftex/updmap/pdftex.map}{/usr/loca
l/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ec-tlf.enc}{/usr/local
/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ot1-tlf.enc}{/usr/local
/texlive/2023basic/texmf-dist/fonts/enc/dvips/tex-gyre/q-ts1.enc}]

Package natbib Warning: Citation `kochukhov21' on page 2 undefined on input lin
e 66.


Package natbib Warning: Citation `kavanagh21' on page 2 undefined on input line
 66.


Package natbib Warning: Citation `kavanagh22' on page 2 undefined on input line
 66.


Package natbib Warning: Citation `vedantham20' on page 2 undefined on input lin
e 68.


Package natbib Warning: Citation `perez-torres21' on page 2 undefined on input 
line 68.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 68.


Package natbib Warning: Citation `pineda23' on page 2 undefined on input line 6
8.


Package natbib Warning: Citation `trigilio23' on page 2 undefined on input line
 68.


Package natbib Warning: Citation `dulk85' on page 2 undefined on input line 68.



Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 68.


Package natbib Warning: Citation `blanco-pozo23' on page 2 undefined on input l
ine 68.


Package natbib Warning: Citation `kavanagh22' on page 2 undefined on input line
 70.


Package natbib Warning: Citation `ashtari22' on page 2 undefined on input line 
70.


Package natbib Warning: Citation `kavanagh19' on page 2 undefined on input line
 70.


Package natbib Warning: Citation `kavanagh22' on page 2 undefined on input line
 72.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 72.


Package natbib Warning: Citation `donati09' on page 2 undefined on input line 7
2.


Package natbib Warning: Citation `kochukhov21' on page 2 undefined on input lin
e 72.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 72.


Package natbib Warning: Citation `morin08' on page 2 undefined on input line 72
.


Package natbib Warning: Citation `lavail18' on page 2 undefined on input line 7
2.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 72.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 74.


Package natbib Warning: Citation `hess11' on page 2 undefined on input line 74.



LaTeX Warning: Reference `sec:expres discusson' on page 2 undefined on input li
ne 74.


Underfull \vbox (badness 6380) has occurred while \output is active

LaTeX Warning: Reference `sec:model' on page 2 undefined on input line 83.


LaTeX Warning: Reference `sec:orbital phases' on page 2 undefined on input line
 83.


LaTeX Warning: Reference `sec:bias' on page 2 undefined on input line 83.


LaTeX Warning: Reference `tab:model parameters' on page 2 undefined on input li
ne 92.


LaTeX Warning: Reference `sec:aligned misaligned' on page 2 undefined on input 
line 94.


Package natbib Warning: Citation `numpy' on page 2 undefined on input line 94.


Package natbib Warning: Citation `numba' on page 2 undefined on input line 94.


LaTeX Warning: Reference `firstpage' on page 2 undefined on input line 133.


LaTeX Warning: Reference `lastpage' on page 2 undefined on input line 133.

[2{/usr/local/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ec-tlf-pc.
enc}]

Package natbib Warning: Citation `donati08' on page 3 undefined on input line 1
34.


Package natbib Warning: Citation `morin08' on page 3 undefined on input line 13
4.


Package natbib Warning: Citation `morin10' on page 3 undefined on input line 13
4.


LaTeX Warning: Reference `sec:star vectors' on page 3 undefined on input line 1
42.


Package natbib Warning: Citation `triaud18' on page 3 undefined on input line 1
50.


LaTeX Warning: Reference `eq:spin orbit angle' on page 3 undefined on input lin
e 150.


LaTeX Warning: Reference `sec:planet vectors' on page 3 undefined on input line
 156.


LaTeX Warning: Reference `fig:sketch geometry' on page 3 undefined on input lin
e 156.


Package natbib Warning: Citation `kivelson95' on page 3 undefined on input line
 172.


LaTeX Warning: Reference `fig:sketch field line' on page 3 undefined on input l
ine 181.


LaTeX Warning: Reference `eq:dipolar field radius' on page 3 undefined on input
 line 188.


LaTeX Warning: Reference `fig:sketch field line' on page 3 undefined on input l
ine 195.


LaTeX Warning: Reference `sec:radio' on page 3 undefined on input line 207.


LaTeX Warning: Reference `eq:field line size' on page 3 undefined on input line
 209.


Package natbib Warning: Citation `kavanagh21' on page 3 undefined on input line
 209.


Package natbib Warning: Citation `kavanagh22' on page 3 undefined on input line
 209.


Package natbib Warning: Citation `marques17' on page 3 undefined on input line 
209.


LaTeX Warning: Reference `firstpage' on page 3 undefined on input line 210.


LaTeX Warning: Reference `lastpage' on page 3 undefined on input line 210.

[3
pdfTeX warning (ext4): destination with the same identifier (name{table.1}) has
 been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.210 
      ]

Package natbib Warning: Citation `alfven42' on page 4 undefined on input line 2
25.


Package natbib Warning: Citation `drell65' on page 4 undefined on input line 22
5.


Package natbib Warning: Citation `treumann06' on page 4 undefined on input line
 225.


Package natbib Warning: Citation `treumann06' on page 4 undefined on input line
 225.


Package natbib Warning: Citation `dulk85' on page 4 undefined on input line 225
.


Underfull \vbox (badness 4954) has occurred while \output is active

LaTeX Warning: Reference `eq:cyclotron frequency' on page 4 undefined on input 
line 234.


LaTeX Warning: Reference `eq:dipolar field radius' on page 4 undefined on input
 line 234.


Package natbib Warning: Citation `kivelson95' on page 4 undefined on input line
 234.


LaTeX Warning: Reference `eq:dipolar field radius' on page 4 undefined on input
 line 241.


LaTeX Warning: Reference `eq:field line strength' on page 4 undefined on input 
line 241.


LaTeX Warning: Reference `firstpage' on page 4 undefined on input line 246.


LaTeX Warning: Reference `lastpage' on page 4 undefined on input line 246.

[4
pdfTeX warning (ext4): destination with the same identifier (name{figure.1}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.246 \end{equation}
                    
pdfTeX warning (ext4): destination with the same identifier (name{figure.2}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.246 \end{equation}
                     <./figs//sketch-geometry.pdf> <./figs//sketch-star-planet-
line.pdf>]

LaTeX Warning: Reference `fig:dipole lines' on page 5 undefined on input line 2
48.


LaTeX Warning: Reference `eq:field line strength - radius' on page 5 undefined 
on input line 250.


LaTeX Warning: Reference `eq:field line strength - radius' on page 5 undefined 
on input line 250.


LaTeX Warning: Reference `sec:newthon method' on page 5 undefined on input line
 257.


LaTeX Warning: Reference `eq:dipolar field radius' on page 5 undefined on input
 line 259.


LaTeX Warning: Reference `sec:field line vector' on page 5 undefined on input l
ine 259.


Package natbib Warning: Citation `kavanagh22' on page 5 undefined on input line
 259.


Package natbib Warning: Citation `das21' on page 5 undefined on input line 266.



LaTeX Warning: Reference `fig:sketch field line' on page 5 undefined on input l
ine 268.


Package natbib Warning: Citation `melrose82' on page 5 undefined on input line 
268.


Package natbib Warning: Citation `lamy22' on page 5 undefined on input line 268
.


Package natbib Warning: Citation `queinnec98' on page 5 undefined on input line
 268.


Package natbib Warning: Citation `pachenko16' on page 5 undefined on input line
 268.


LaTeX Warning: Reference `sec:dipole' on page 5 undefined on input line 270.


LaTeX Warning: Reference `eq:cyclotron frequency' on page 5 undefined on input 
line 272.


LaTeX Warning: Reference `eq:field line strength - radius' on page 5 undefined 
on input line 272.


LaTeX Warning: Reference `eq:field line size' on page 5 undefined on input line
 279.


Package natbib Warning: Citation `bigg64' on page 5 undefined on input line 308
.


Package natbib Warning: Citation `perez-torres21' on page 5 undefined on input 
line 308.


Package natbib Warning: Citation `kavanagh22' on page 5 undefined on input line
 308.


LaTeX Warning: Reference `firstpage' on page 5 undefined on input line 314.


LaTeX Warning: Reference `lastpage' on page 5 undefined on input line 314.

[5
pdfTeX warning (ext4): destination with the same identifier (name{figure.3}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.314 \subsection
                 {The expectation of emission at quadrature} <./figs//field-lin
es.pdf>]

LaTeX Warning: Reference `sec:star vectors' on page 6 undefined on input line 3
17.


LaTeX Warning: Reference `sec:planet vectors' on page 6 undefined on input line
 317.


LaTeX Warning: Reference `eq:Br' on page 6 undefined on input line 329.


LaTeX Warning: Reference `eq:theta hat' on page 6 undefined on input line 329.


LaTeX Warning: Reference `eq:beam angle' on page 6 undefined on input line 329.



LaTeX Warning: Reference `eq:Br' on page 6 undefined on input line 329.


LaTeX Warning: Reference `eq:theta hat' on page 6 undefined on input line 329.


LaTeX Warning: Reference `eq:quadrature angle' on page 6 undefined on input lin
e 336.


LaTeX Warning: Reference `fig:quadrature angles' on page 6 undefined on input l
ine 336.


LaTeX Warning: Reference `eq:quadrature angle' on page 6 undefined on input lin
e 343.


LaTeX Warning: Reference `eq:quadrature angle' on page 6 undefined on input lin
e 343.


LaTeX Warning: Reference `fig:quadrature' on page 6 undefined on input line 356
.


LaTeX Warning: Reference `sec:quadrature' on page 6 undefined on input line 356
.


LaTeX Warning: Reference `tab:quadrature values' on page 6 undefined on input l
ine 356.


LaTeX Warning: Reference `eq:fmax' on page 6 undefined on input line 356.


LaTeX Warning: Reference `eq:fplanet' on page 6 undefined on input line 356.


LaTeX Warning: Reference `fig:quadrature' on page 6 undefined on input line 358
.


LaTeX Warning: Reference `sec:quadrature' on page 6 undefined on input line 358
.


LaTeX Warning: Reference `firstpage' on page 6 undefined on input line 359.


LaTeX Warning: Reference `lastpage' on page 6 undefined on input line 359.

[6
pdfTeX warning (ext4): destination with the same identifier (name{figure.4}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.359 
       <./figs//quadrature-angles.pdf>]

LaTeX Warning: Reference `tab:quadrature values' on page 7 undefined on input l
ine 360.


LaTeX Warning: Reference `fig:quadrature pdf' on page 7 undefined on input line
 360.


Package natbib Warning: Citation `marques17' on page 7 undefined on input line 
362.


LaTeX Warning: Reference `sec:io' on page 7 undefined on input line 362.


Package natbib Warning: Citation `marques17' on page 7 undefined on input line 
362.


LaTeX Warning: Reference `fig:quadrature' on page 7 undefined on input line 365
.


LaTeX Warning: Reference `fig:quadrature pdf' on page 7 undefined on input line
 365.


LaTeX Warning: Reference `fig:quadrature' on page 7 undefined on input line 365
.


LaTeX Warning: Reference `fig:quadrature pdf' on page 7 undefined on input line
 365.


LaTeX Warning: Reference `tab:quadrature values' on page 7 undefined on input l
ine 394.


LaTeX Warning: Reference `tab:quadrature values' on page 7 undefined on input l
ine 394.


LaTeX Warning: Reference `tab:quadrature values' on page 7 undefined on input l
ine 411.


LaTeX Warning: Reference `sec:aligned misaligned' on page 7 undefined on input 
line 411.


LaTeX Warning: Reference `fig:pdf angles' on page 7 undefined on input line 411
.


Underfull \vbox (badness 10000) has occurred while \output is active

LaTeX Warning: Reference `firstpage' on page 7 undefined on input line 413.


LaTeX Warning: Reference `lastpage' on page 7 undefined on input line 413.

[7
pdfTeX warning (ext4): destination with the same identifier (name{table.2}) has
 been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.413 W
       e see that apart from the projected spin-orbit angle, when the values...

pdfTeX warning (ext4): destination with the same identifier (name{figure.5}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.413 W
       e see that apart from the projected spin-orbit angle, when the values...

pdfTeX warning (ext4): destination with the same identifier (name{figure.6}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.413 W
       e see that apart from the projected spin-orbit angle, when the values...
 <./figs//quadrature-lc.pdf> <./figs//quadrature-pd.pdf>]

LaTeX Warning: Reference `tab:quadrature values' on page 8 undefined on input l
ine 415.


Package natbib Warning: Citation `hess11' on page 8 undefined on input line 415
.


LaTeX Warning: Reference `fig:quadrature pdf' on page 8 undefined on input line
 420.


LaTeX Warning: Reference `tab:quadrature values' on page 8 undefined on input l
ine 420.


LaTeX Warning: Reference `fig:quadrature pdf' on page 8 undefined on input line
 420.


LaTeX Warning: Reference `tab:quadrature values' on page 8 undefined on input l
ine 420.


Package natbib Warning: Citation `callingham21b' on page 8 undefined on input l
ine 431.


LaTeX Warning: Reference `tab:model parameters' on page 8 undefined on input li
ne 433.


Package natbib Warning: Citation `winters19' on page 8 undefined on input line 
442.


Package natbib Warning: Citation `winters19' on page 8 undefined on input line 
442.


Package natbib Warning: Citation `schweitzer19' on page 8 undefined on input li
ne 442.


LaTeX Warning: Reference `eq:mass-radius relation' on page 8 undefined on input
 line 449.


LaTeX Warning: Reference `eq:mass-radius relation' on page 8 undefined on input
 line 449.


Package natbib Warning: Citation `schweitzer19' on page 8 undefined on input li
ne 449.


Package natbib Warning: Citation `popinchalk21' on page 8 undefined on input li
ne 451.


Package natbib Warning: Citation `lu22' on page 8 undefined on input line 451.


Package natbib Warning: Citation `lu22' on page 8 undefined on input line 451.


Package natbib Warning: Citation `reinhold19' on page 8 undefined on input line
 451.


Package natbib Warning: Citation `popinchalk21' on page 8 undefined on input li
ne 451.


Package natbib Warning: Citation `popinchalk21' on page 8 undefined on input li
ne 451.


Package natbib Warning: Citation `donati08' on page 8 undefined on input line 4
53.


Package natbib Warning: Citation `morin08' on page 8 undefined on input line 45
3.


Package natbib Warning: Citation `morin10' on page 8 undefined on input line 45
3.


Package natbib Warning: Citation `lehmann19' on page 8 undefined on input line 
453.


Package natbib Warning: Citation `lehmann21' on page 8 undefined on input line 
453.


Package natbib Warning: Citation `lehmann19' on page 8 undefined on input line 
453.


Package natbib Warning: Citation `rappaport13' on page 8 undefined on input lin
e 455.


Package natbib Warning: Citation `unterborn19' on page 8 undefined on input lin
e 461.


Underfull \vbox (badness 10000) has occurred while \output is active

LaTeX Warning: Reference `firstpage' on page 8 undefined on input line 465.


LaTeX Warning: Reference `lastpage' on page 8 undefined on input line 465.

[8]

Package natbib Warning: Citation `kavanagh22' on page 9 undefined on input line
 469.


Package natbib Warning: Citation `shulyak17' on page 9 undefined on input line 
469.


Package natbib Warning: Citation `kavanagh22' on page 9 undefined on input line
 469.


Package natbib Warning: Citation `schlecker22' on page 9 undefined on input lin
e 471.


Package natbib Warning: Citation `ribas23' on page 9 undefined on input line 47
1.


Package natbib Warning: Citation `stefansson22' on page 9 undefined on input li
ne 473.


Package natbib Warning: Citation `albrecht22' on page 9 undefined on input line
 473.


Underfull \vbox (badness 10000) has occurred while \output is active

LaTeX Warning: Reference `firstpage' on page 9 undefined on input line 475.


LaTeX Warning: Reference `lastpage' on page 9 undefined on input line 475.

[9
pdfTeX warning (ext4): destination with the same identifier (name{figure.7}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.475 T
       he final set of values to sample relate to the emission. For fundamen...
 <./figs//prob-density-2d.pdf>]

LaTeX Warning: Reference `eq:cyclotron frequency' on page 10 undefined on input
 line 475.


Package natbib Warning: Citation `edler21' on page 10 undefined on input line 4
75.


LaTeX Warning: Reference `sec:radio' on page 10 undefined on input line 477.


LaTeX Warning: Reference `sec:samples' on page 10 undefined on input line 494.


LaTeX Warning: Reference `sec:scatter plots' on page 10 undefined on input line
 496.


LaTeX Warning: Reference `fig:scatter star' on page 10 undefined on input line 
505.


LaTeX Warning: Reference `fig:scatter star' on page 10 undefined on input line 
507.


LaTeX Warning: Reference `eq:z_s' on page 10 undefined on input line 507.


LaTeX Warning: Reference `eq:z_B' on page 10 undefined on input line 507.


LaTeX Warning: Reference `fig:scatter star' on page 10 undefined on input line 
514.


LaTeX Warning: Reference `eq:magnetic axis inclination' on page 10 undefined on
 input line 516.


LaTeX Warning: Reference `sec:samples' on page 10 undefined on input line 516.


LaTeX Warning: Reference `fig:scatter star' on page 10 undefined on input line 
532.


LaTeX Warning: Reference `fig:planet hists' on page 10 undefined on input line 
532.


LaTeX Warning: Reference `fig:c1-c2' on page 10 undefined on input line 532.


LaTeX Warning: Reference `firstpage' on page 10 undefined on input line 534.


LaTeX Warning: Reference `lastpage' on page 10 undefined on input line 534.

[10]
Underfull \vbox (badness 4543) has occurred while \output is active

LaTeX Warning: Reference `fig:c1-c2' on page 11 undefined on input line 545.


LaTeX Warning: Reference `eq:polar orbits' on page 11 undefined on input line 5
45.


LaTeX Warning: Reference `eq:beam angle' on page 11 undefined on input line 547
.


LaTeX Warning: Reference `eq:polar orbits' on page 11 undefined on input line 5
60.


LaTeX Warning: Reference `fig:c1-c2' on page 11 undefined on input line 560.


LaTeX Warning: Reference `eq:beam angle radial field lines' on page 11 undefine
d on input line 574.


LaTeX Warning: Reference `fig:c1-c2' on page 11 undefined on input line 574.


Package natbib Warning: Citation `villadsen19' on page 11 undefined on input li
ne 576.


LaTeX Warning: Reference `firstpage' on page 11 undefined on input line 577.


LaTeX Warning: Reference `lastpage' on page 11 undefined on input line 577.

[11
pdfTeX warning (ext4): destination with the same identifier (name{figure.8}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.577 
       <./figs//scatter-star.pdf>]

LaTeX Warning: Reference `fig:scatter plots' on page 12 undefined on input line
 578.


LaTeX Warning: Reference `tab:quadrature values' on page 12 undefined on input 
line 590.


LaTeX Warning: Reference `tab:quadrature values' on page 12 undefined on input 
line 590.


LaTeX Warning: Reference `sec:optimal - planet' on page 12 undefined on input l
ine 597.


LaTeX Warning: Reference `sec:optimal - planet' on page 12 undefined on input l
ine 597.


LaTeX Warning: Reference `fig:scatter plots' on page 12 undefined on input line
 607.


LaTeX Warning: Reference `sec:optimal - star' on page 12 undefined on input lin
e 609.


LaTeX Warning: Reference `sec:optimal - planet' on page 12 undefined on input l
ine 609.


Package natbib Warning: Citation `hinkley23' on page 12 undefined on input line
 618.


Package natbib Warning: Citation `gaspar16' on page 12 undefined on input line 
618.


Package natbib Warning: Citation `fares12' on page 12 undefined on input line 6
18.


Package natbib Warning: Citation `jeffers18' on page 12 undefined on input line
 618.


Package natbib Warning: Citation `seach22' on page 12 undefined on input line 6
18.


Package natbib Warning: Citation `perryman14' on page 12 undefined on input lin
e 620.


Package natbib Warning: Citation `winn22' on page 12 undefined on input line 62
0.


Package natbib Warning: Citation `curiel22' on page 12 undefined on input line 
620.


Package natbib Warning: Citation `morin08' on page 12 undefined on input line 6
20.


LaTeX Warning: Reference `sec:samples' on page 12 undefined on input line 622.


LaTeX Warning: Reference `fig:c1-c2' on page 12 undefined on input line 624.


LaTeX Warning: Reference `fig:scatter star' on page 12 undefined on input line 
624.


LaTeX Warning: Reference `fig:scatter plots' on page 12 undefined on input line
 624.


LaTeX Warning: Reference `firstpage' on page 12 undefined on input line 625.


LaTeX Warning: Reference `lastpage' on page 12 undefined on input line 625.

[12
pdfTeX warning (ext4): destination with the same identifier (name{figure.9}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.625 
       <./figs//planet-hists.pdf>]

Package natbib Warning: Citation `kavanagh21' on page 13 undefined on input lin
e 636.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 636.


Package natbib Warning: Citation `saur13' on page 13 undefined on input line 63
6.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 636.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 638.


Package natbib Warning: Citation `kavanagh21' on page 13 undefined on input lin
e 638.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 638.


Package natbib Warning: Citation `hess10' on page 13 undefined on input line 63
8.


Package natbib Warning: Citation `lehmann22' on page 13 undefined on input line
 640.


Package natbib Warning: Citation `jardine02' on page 13 undefined on input line
 640.


Package natbib Warning: Citation `llama18' on page 13 undefined on input line 6
42.


Package natbib Warning: Citation `owocki22' on page 13 undefined on input line 
642.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 642.


Underfull \vbox (badness 10000) has occurred while \output is active

LaTeX Warning: Reference `firstpage' on page 13 undefined on input line 643.


LaTeX Warning: Reference `lastpage' on page 13 undefined on input line 643.

[13
pdfTeX warning (ext4): destination with the same identifier (name{figure.10}) h
as been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.643 
       <./figs//c1-c2.pdf>]

Package natbib Warning: Citation `hess11' on page 14 undefined on input line 65
1.


Package natbib Warning: Citation `louis19' on page 14 undefined on input line 6
51.


Package natbib Warning: Citation `kavanagh22' on page 14 undefined on input lin
e 659.


Package natbib Warning: Citation `morin08' on page 14 undefined on input line 6
65.


Package natbib Warning: Citation `morin10' on page 14 undefined on input line 6
65.


Package natbib Warning: Citation `lavail18' on page 14 undefined on input line 
665.


Package natbib Warning: Citation `callingham21b' on page 14 undefined on input 
line 667.


LaTeX Warning: Reference `sec:transiting' on page 14 undefined on input line 66
7.


LaTeX Warning: Reference `firstpage' on page 14 undefined on input line 668.


LaTeX Warning: Reference `lastpage' on page 14 undefined on input line 668.

[14
pdfTeX warning (ext4): destination with the same identifier (name{figure.11}) h
as been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.668 
       <./figs//sketch-c1.pdf>]

LaTeX Warning: Reference `sec:io' on page 15 undefined on input line 669.


Package natbib Warning: Citation `shkolnik03' on page 15 undefined on input lin
e 669.


Package natbib Warning: Citation `lanza09' on page 15 undefined on input line 6
69.


Package natbib Warning: Citation `klein22' on page 15 undefined on input line 6
69.


LaTeX Warning: Reference `sec:model' on page 15 undefined on input line 685.

No file main.bbl.

LaTeX Warning: Reference `fig:star vectors' on page 15 undefined on input line 
731.


LaTeX Warning: Reference `fig:planet vectors' on page 15 undefined on input lin
e 781.


LaTeX Warning: Reference `EQ:DIPOLAR FIELD LINE SOLVE' on page 15 undefined on 
input line 794.


LaTeX Warning: Reference `EQ:DIPOLAR FIELD LINE SOLVE' on page 15 undefined on 
input line 797.


LaTeX Warning: Reference `EQ:DIPOLAR FIELD LINE SOLVE' on page 15 undefined on 
input line 797.


LaTeX Warning: Reference `firstpage' on page 15 undefined on input line 808.


LaTeX Warning: Reference `lastpage' on page 15 undefined on input line 808.

[15
pdfTeX warning (ext4): destination with the same identifier (name{figure.A1.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.808 \end{equation}
                     <./figs//sketch-vectors-star.pdf>]

LaTeX Warning: Reference `EQ:DIPOLAR FIELD LINE SOLVE' on page 16 undefined on 
input line 810.


LaTeX Warning: Reference `eq:dipolar field radius' on page 16 undefined on inpu
t line 810.


Package natbib Warning: Citation `kivelson95' on page 16 undefined on input lin
e 826.


LaTeX Warning: Reference `fig:sketch field line' on page 16 undefined on input 
line 833.


LaTeX Warning: Reference `fig:emitting field vectors' on page 16 undefined on i
nput line 833.


LaTeX Warning: Reference `sec:quadrature' on page 16 undefined on input line 85
6.


Package natbib Warning: Citation `marques17' on page 16 undefined on input line
 856.


LaTeX Warning: Reference `tab:jupiter io' on page 16 undefined on input line 85
6.


LaTeX Warning: Reference `fig:io' on page 16 undefined on input line 858.


Package natbib Warning: Citation `marques17' on page 16 undefined on input line
 858.


LaTeX Warning: Reference `tab:jupiter io' on page 16 undefined on input line 85
8.


LaTeX Warning: Reference `tab:quadrature values' on page 16 undefined on input 
line 858.


LaTeX Warning: Reference `sec:radio' on page 16 undefined on input line 858.


Package natbib Warning: Citation `marques17' on page 16 undefined on input line
 860.


Package natbib Warning: Citation `marques17' on page 16 undefined on input line
 860.


Package natbib Warning: Citation `bagenal13' on page 16 undefined on input line
 882.


Package natbib Warning: Citation `bagenal20' on page 16 undefined on input line
 882.


Package natbib Warning: Citation `bills22' on page 16 undefined on input line 8
82.


Package natbib Warning: Citation `marques17' on page 16 undefined on input line
 889.


Package natbib Warning: Citation `marques17' on page 16 undefined on input line
 889.


LaTeX Warning: Reference `sec:geometry' on page 16 undefined on input line 889.



Package natbib Warning: Citation `connerney22' on page 16 undefined on input li
ne 889.


Package natbib Warning: Citation `marques17' on page 16 undefined on input line
 889.


Package natbib Warning: Citation `marques17' on page 16 undefined on input line
 889.


LaTeX Warning: Reference `sec:geometry' on page 16 undefined on input line 889.



Package natbib Warning: Citation `connerney22' on page 16 undefined on input li
ne 889.


LaTeX Warning: Reference `fig:scatter plots' on page 16 undefined on input line
 900.


LaTeX Warning: Reference `sec:bias general' on page 16 undefined on input line 
900.


LaTeX Warning: Reference `sec:samples' on page 16 undefined on input line 904.


LaTeX Warning: Reference `sec:samples' on page 16 undefined on input line 904.


LaTeX Warning: Reference `firstpage' on page 16 undefined on input line 906.


LaTeX Warning: Reference `lastpage' on page 16 undefined on input line 906.

[16
pdfTeX warning (ext4): destination with the same identifier (name{figure.A2.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.906 \end{figure*}
                   
pdfTeX warning (ext4): destination with the same identifier (name{figure.A4.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.906 \end{figure*}
                   
pdfTeX warning (ext4): destination with the same identifier (name{table.A5.1}) 
has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.906 \end{figure*}
                    <./figs//sketch-vectors-planet.pdf> <./figs//sketch-vectors
-cone.pdf>]

Package natbib Warning: There were undefined citations.


LaTeX Warning: Reference `firstpage' on page 17 undefined on input line 913.


LaTeX Warning: Reference `lastpage' on page 17 undefined on input line 913.

[17
pdfTeX warning (ext4): destination with the same identifier (name{figure.A5.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.913 \end{document}
                     <./figs//io.pdf>]
Underfull \vbox (badness 10000) has occurred while \output is active

LaTeX Warning: Reference `firstpage' on page 18 undefined on input line 913.


LaTeX Warning: Reference `lastpage' on page 18 undefined on input line 913.

[18
pdfTeX warning (ext4): destination with the same identifier (name{figure.A6.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.913 \end{document}
                     <./figs//scatter-plots.pdf>] (aux/main.aux)

LaTeX Font Warning: Size substitutions with differences
(Font)              up to 0.5pt have occurred.


LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package rerunfilecheck Warning: File `main.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.

 )
(see the transcript file for additional information)
pdfTeX warning (dest): name{Hfootnote.1} has been referenced but does not exist
, replaced by a fixed one

</usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI5.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI7.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.p
fb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi
7.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/c
mr10.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/c
m/cmr5.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts
/cm/cmsy10.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsf
onts/cm/cmsy7.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/a
msfonts/cm/cmtt8.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/publi
c/tex-gyre/qtmr.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public
/newtx/txexs.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/ne
wtx/txmiaX.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/txfo
nts/txsya.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx
/txsys.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/zt
mb.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/ztmr.p
fb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/ztmri.pfb>
Output written on aux/main.pdf (18 pages, 5083356 bytes).
Transcript written on aux/main.log.
This is BibTeX, Version 0.99d (TeX Live 2023)
The top-level auxiliary file: aux/main.aux
The style file: mnras.bst
Database file #1: bibliography.bib
Repeated entry---line 250 of file bibliography.bib
 : @incollection{bagenal13
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 852 of file bibliography.bib
 : @article{morin08
 :                 ,
I'm skipping whatever remains of this entry
Repeated entry---line 955 of file bibliography.bib
 : @article{klein22
 :                 ,
I'm skipping whatever remains of this entry
Repeated entry---line 988 of file bibliography.bib
 : @article{lanza09
 :                 ,
I'm skipping whatever remains of this entry
Warning--empty publisher in bagenal13
Warning--empty publisher in triaud18
(There were 4 error messages)
This is pdfTeX, Version 3.141592653-2.6-1.40.25 (TeX Live 2023) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2022-11-01> patch level 1
L3 programming layer <2023-02-22> (./mnras.cls
Document Class: mnras 2015/05/22\ v3.0\ LaTeX2e MNRAS document class
MNRAS document style v3.0, released 2015/05/22
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.
sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
 (/usr/local/texlive/2023basic/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/gettitlestring/gettitlestr
ing.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/kvoptions/kvoptions.sty)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty)
) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/atbegshi-ltx.sty)

Package hyperref Warning: Option `pdfpagelabels' is turned off
(hyperref)                because \thepage is undefined.

) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/rerunfilecheck/rerunfilechec
k.sty (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/atveryend-ltx.sty
)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/uniquecounter/uniquecounte
r.sty))) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/natbib/natbib.sty))
 (/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/newtxtext.sty
`newtxtext' v1.71, 2022/02/28 Text macros taking advantage of TeXGyre Termes an
d its extensions (msharpe)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/textcomp.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/carlisle/scalefnt.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kastrup/binhex.tex)
ntx@otftextfalse
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/fontaxes/fontaxes.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.71, 2022/01/16 Math macros based originally on txfonts (msharpe)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifxetex.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifluatex.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kastrup/binhex.tex)
amsthm NOT loaded
) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fontenc.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1minntx.fd))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/ae.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fontenc.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/aecompl.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/mathcolor.ltx))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1ntxtlf.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/l3backend/l3backend-pdftex.d
ef) (aux/main.aux)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/omlntxmi.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(aux/main.out) (aux/main.out)
(/usr/local/texlive/2023basic/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.s
ty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg
)) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/ot1minntx.fd)

LaTeX Font Warning: Font shape `OML/cmm/b/it' in size <10.5> not available
(Font)              size <10.95> substituted on input line 34.

(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/ueur.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxsyc.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1ntxsups.fd)

LaTeX Font Warning: Font shape `OML/cmm/b/it' in size <5.5> not available
(Font)              size <5> substituted on input line 34.

(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/t1aett.fd)

Package natbib Warning: Citation `nicholson19' on page 1 undefined on input lin
e 54.


Package natbib Warning: Citation `burn21' on page 1 undefined on input line 54.



Package natbib Warning: Citation `winters19' on page 1 undefined on input line 
54.


Package natbib Warning: Citation `burn21' on page 1 undefined on input line 54.



Package natbib Warning: Citation `schlecker22' on page 1 undefined on input lin
e 54.


Package natbib Warning: Citation `zarka07' on page 1 undefined on input line 56
.


Package natbib Warning: Citation `saur13' on page 1 undefined on input line 56.



Package natbib Warning: Citation `alfven42' on page 1 undefined on input line 5
6.


Package natbib Warning: Citation `neubauer80' on page 1 undefined on input line
 56.


Package natbib Warning: Citation `dulk85' on page 1 undefined on input line 56.



Package natbib Warning: Citation `treumann06' on page 1 undefined on input line
 56.


Package natbib Warning: Citation `vidotto14' on page 1 undefined on input line 
64.

(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/ts1ntxtlf.fd) [1{/usr/
local/texlive/2023basic/texmf-var/fonts/map/pdftex/updmap/pdftex.map}{/usr/loca
l/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ec-tlf.enc}{/usr/local
/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ot1-tlf.enc}{/usr/local
/texlive/2023basic/texmf-dist/fonts/enc/dvips/tex-gyre/q-ts1.enc}]

Package natbib Warning: Citation `kochukhov21' on page 2 undefined on input lin
e 66.


Package natbib Warning: Citation `kavanagh21' on page 2 undefined on input line
 66.


Package natbib Warning: Citation `kavanagh22' on page 2 undefined on input line
 66.


Package natbib Warning: Citation `vedantham20' on page 2 undefined on input lin
e 68.


Package natbib Warning: Citation `perez-torres21' on page 2 undefined on input 
line 68.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 68.


Package natbib Warning: Citation `pineda23' on page 2 undefined on input line 6
8.


Package natbib Warning: Citation `trigilio23' on page 2 undefined on input line
 68.


Package natbib Warning: Citation `dulk85' on page 2 undefined on input line 68.



Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 68.


Package natbib Warning: Citation `blanco-pozo23' on page 2 undefined on input l
ine 68.


Package natbib Warning: Citation `kavanagh22' on page 2 undefined on input line
 70.


Package natbib Warning: Citation `ashtari22' on page 2 undefined on input line 
70.


Package natbib Warning: Citation `kavanagh19' on page 2 undefined on input line
 70.


Package natbib Warning: Citation `kavanagh22' on page 2 undefined on input line
 72.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 72.


Package natbib Warning: Citation `donati09' on page 2 undefined on input line 7
2.


Package natbib Warning: Citation `kochukhov21' on page 2 undefined on input lin
e 72.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 72.


Package natbib Warning: Citation `morin08' on page 2 undefined on input line 72
.


Package natbib Warning: Citation `lavail18' on page 2 undefined on input line 7
2.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 72.


Package natbib Warning: Citation `callingham21b' on page 2 undefined on input l
ine 74.


Package natbib Warning: Citation `hess11' on page 2 undefined on input line 74.



Underfull \vbox (badness 6380) has occurred while \output is active

Package natbib Warning: Citation `numpy' on page 2 undefined on input line 94.


Package natbib Warning: Citation `numba' on page 2 undefined on input line 94.

[2{/usr/local/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ec-tlf-pc.
enc}]

Package natbib Warning: Citation `donati08' on page 3 undefined on input line 1
34.


Package natbib Warning: Citation `morin08' on page 3 undefined on input line 13
4.


Package natbib Warning: Citation `morin10' on page 3 undefined on input line 13
4.


Package natbib Warning: Citation `triaud18' on page 3 undefined on input line 1
50.


Package natbib Warning: Citation `kivelson95' on page 3 undefined on input line
 172.


Package natbib Warning: Citation `kavanagh21' on page 3 undefined on input line
 209.


Package natbib Warning: Citation `kavanagh22' on page 3 undefined on input line
 209.


Package natbib Warning: Citation `marques17' on page 3 undefined on input line 
209.

[3
pdfTeX warning (ext4): destination with the same identifier (name{table.1}) has
 been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.210 
      ]

Package natbib Warning: Citation `alfven42' on page 4 undefined on input line 2
25.


Package natbib Warning: Citation `drell65' on page 4 undefined on input line 22
5.


Package natbib Warning: Citation `treumann06' on page 4 undefined on input line
 225.


Package natbib Warning: Citation `treumann06' on page 4 undefined on input line
 225.


Package natbib Warning: Citation `dulk85' on page 4 undefined on input line 225
.


Underfull \vbox (badness 1077) has occurred while \output is active

Package natbib Warning: Citation `kivelson95' on page 4 undefined on input line
 234.

[4
pdfTeX warning (ext4): destination with the same identifier (name{figure.1}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.246 \end{equation}
                    
pdfTeX warning (ext4): destination with the same identifier (name{figure.2}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.246 \end{equation}
                     <./figs//sketch-geometry.pdf> <./figs//sketch-star-planet-
line.pdf>]

Package natbib Warning: Citation `kavanagh22' on page 5 undefined on input line
 259.


Package natbib Warning: Citation `das21' on page 5 undefined on input line 266.



Package natbib Warning: Citation `melrose82' on page 5 undefined on input line 
268.


Package natbib Warning: Citation `lamy22' on page 5 undefined on input line 268
.


Package natbib Warning: Citation `queinnec98' on page 5 undefined on input line
 268.


Package natbib Warning: Citation `pachenko16' on page 5 undefined on input line
 268.


Package natbib Warning: Citation `bigg64' on page 5 undefined on input line 308
.


Package natbib Warning: Citation `perez-torres21' on page 5 undefined on input 
line 308.


Package natbib Warning: Citation `kavanagh22' on page 5 undefined on input line
 308.

[5
pdfTeX warning (ext4): destination with the same identifier (name{figure.3}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.314 \subsection
                 {The expectation of emission at quadrature} <./figs//field-lin
es.pdf>] [6
pdfTeX warning (ext4): destination with the same identifier (name{figure.4}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.359 
       <./figs//quadrature-angles.pdf>]

Package natbib Warning: Citation `marques17' on page 7 undefined on input line 
362.


Package natbib Warning: Citation `marques17' on page 7 undefined on input line 
362.

[7
pdfTeX warning (ext4): destination with the same identifier (name{table.2}) has
 been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.414 
      
pdfTeX warning (ext4): destination with the same identifier (name{figure.5}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.414 
      
pdfTeX warning (ext4): destination with the same identifier (name{figure.6}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.414 
       <./figs//quadrature-lc.pdf> <./figs//quadrature-pd.pdf>]

Package natbib Warning: Citation `hess11' on page 8 undefined on input line 415
.


Package natbib Warning: Citation `callingham21b' on page 8 undefined on input l
ine 431.


Package natbib Warning: Citation `winters19' on page 8 undefined on input line 
442.


Package natbib Warning: Citation `winters19' on page 8 undefined on input line 
442.


Package natbib Warning: Citation `schweitzer19' on page 8 undefined on input li
ne 442.


Package natbib Warning: Citation `schweitzer19' on page 8 undefined on input li
ne 449.


Package natbib Warning: Citation `popinchalk21' on page 8 undefined on input li
ne 451.


Package natbib Warning: Citation `lu22' on page 8 undefined on input line 451.


Package natbib Warning: Citation `lu22' on page 8 undefined on input line 451.


Package natbib Warning: Citation `reinhold19' on page 8 undefined on input line
 451.


Package natbib Warning: Citation `popinchalk21' on page 8 undefined on input li
ne 451.


Package natbib Warning: Citation `popinchalk21' on page 8 undefined on input li
ne 451.


Package natbib Warning: Citation `donati08' on page 8 undefined on input line 4
53.


Package natbib Warning: Citation `morin08' on page 8 undefined on input line 45
3.


Package natbib Warning: Citation `morin10' on page 8 undefined on input line 45
3.


Package natbib Warning: Citation `lehmann19' on page 8 undefined on input line 
453.


Package natbib Warning: Citation `lehmann21' on page 8 undefined on input line 
453.


Package natbib Warning: Citation `lehmann19' on page 8 undefined on input line 
453.


Package natbib Warning: Citation `rappaport13' on page 8 undefined on input lin
e 455.


Package natbib Warning: Citation `unterborn19' on page 8 undefined on input lin
e 461.


Package natbib Warning: Citation `kavanagh22' on page 8 undefined on input line
 469.


Package natbib Warning: Citation `shulyak17' on page 8 undefined on input line 
469.


Package natbib Warning: Citation `kavanagh22' on page 8 undefined on input line
 469.

[8]

Package natbib Warning: Citation `schlecker22' on page 9 undefined on input lin
e 471.


Package natbib Warning: Citation `ribas23' on page 9 undefined on input line 47
1.


Underfull \vbox (badness 10000) has occurred while \output is active

Package natbib Warning: Citation `stefansson22' on page 9 undefined on input li
ne 473.


Package natbib Warning: Citation `albrecht22' on page 9 undefined on input line
 473.


Package natbib Warning: Citation `edler21' on page 9 undefined on input line 47
5.


Underfull \vbox (badness 10000) has occurred while \output is active [9
pdfTeX warning (ext4): destination with the same identifier (name{figure.7}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.476 
       <./figs//prob-density-2d.pdf>] [10]

Package natbib Warning: Citation `villadsen19' on page 11 undefined on input li
ne 576.

[11
pdfTeX warning (ext4): destination with the same identifier (name{figure.8}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.579 
       <./figs//scatter-star.pdf>]

Package natbib Warning: Citation `hinkley23' on page 12 undefined on input line
 618.


Package natbib Warning: Citation `gaspar16' on page 12 undefined on input line 
618.


Package natbib Warning: Citation `fares12' on page 12 undefined on input line 6
18.


Package natbib Warning: Citation `jeffers18' on page 12 undefined on input line
 618.


Package natbib Warning: Citation `seach22' on page 12 undefined on input line 6
18.


Underfull \vbox (badness 2409) has occurred while \output is active

Package natbib Warning: Citation `perryman14' on page 12 undefined on input lin
e 620.


Package natbib Warning: Citation `winn22' on page 12 undefined on input line 62
0.


Package natbib Warning: Citation `curiel22' on page 12 undefined on input line 
620.


Package natbib Warning: Citation `morin08' on page 12 undefined on input line 6
20.


Underfull \vbox (badness 10000) has occurred while \output is active [12
pdfTeX warning (ext4): destination with the same identifier (name{figure.9}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.634 \subsection
                 {Current limitations to the model} <./figs//planet-hists.pdf>]

Package natbib Warning: Citation `kavanagh21' on page 13 undefined on input lin
e 636.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 636.


Package natbib Warning: Citation `saur13' on page 13 undefined on input line 63
6.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 636.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 638.


Package natbib Warning: Citation `kavanagh21' on page 13 undefined on input lin
e 638.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 638.


Package natbib Warning: Citation `hess10' on page 13 undefined on input line 63
8.


Package natbib Warning: Citation `lehmann22' on page 13 undefined on input line
 640.


Package natbib Warning: Citation `jardine02' on page 13 undefined on input line
 640.


Package natbib Warning: Citation `llama18' on page 13 undefined on input line 6
42.


Package natbib Warning: Citation `owocki22' on page 13 undefined on input line 
642.


Package natbib Warning: Citation `kavanagh22' on page 13 undefined on input lin
e 642.


Underfull \vbox (badness 10000) has occurred while \output is active [13
pdfTeX warning (ext4): destination with the same identifier (name{figure.10}) h
as been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.643 
       <./figs//c1-c2.pdf>]

Package natbib Warning: Citation `hess11' on page 14 undefined on input line 65
1.


Package natbib Warning: Citation `louis19' on page 14 undefined on input line 6
51.


Package natbib Warning: Citation `kavanagh22' on page 14 undefined on input lin
e 659.


Underfull \vbox (badness 1859) has occurred while \output is active

Package natbib Warning: Citation `morin08' on page 14 undefined on input line 6
65.


Package natbib Warning: Citation `morin10' on page 14 undefined on input line 6
65.


Package natbib Warning: Citation `lavail18' on page 14 undefined on input line 
665.


Package natbib Warning: Citation `callingham21b' on page 14 undefined on input 
line 667.


Underfull \vbox (badness 10000) has occurred while \output is active [14
pdfTeX warning (ext4): destination with the same identifier (name{figure.11}) h
as been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.668 
       <./figs//sketch-c1.pdf>]

Package natbib Warning: Citation `shkolnik03' on page 15 undefined on input lin
e 669.


Package natbib Warning: Citation `lanza09' on page 15 undefined on input line 6
69.


Package natbib Warning: Citation `klein22' on page 15 undefined on input line 6
69.

(aux/main.bbl
Underfull \hbox (badness 1122) in paragraph at lines 202--207
\T1/ntxtlf/m/n/8 ond Work-shop on the LLVM Com-piler In-fras-truc-ture in HPC.

Package hyperref Warning: Suppressing empty link on input line 321.

[15]) [16
pdfTeX warning (ext4): destination with the same identifier (name{figure.A1.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.816 \section
              {The magnetic field vector along the field line}
pdfTeX warning (ext4): destination with the same identifier (name{figure.A2.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.816 \section
              {The magnetic field vector along the field line} <./figs//sketch-
vectors-star.pdf> <./figs//sketch-vectors-planet.pdf>]

Package natbib Warning: Citation `kivelson95' on page 17 undefined on input lin
e 826.


Package natbib Warning: Citation `marques17' on page 17 undefined on input line
 856.


Package natbib Warning: Citation `marques17' on page 17 undefined on input line
 858.


Package natbib Warning: Citation `marques17' on page 17 undefined on input line
 860.


Package natbib Warning: Citation `marques17' on page 17 undefined on input line
 860.


Package natbib Warning: Citation `bagenal13' on page 17 undefined on input line
 882.


Package natbib Warning: Citation `bagenal20' on page 17 undefined on input line
 882.


Package natbib Warning: Citation `bills22' on page 17 undefined on input line 8
82.


Package natbib Warning: Citation `marques17' on page 17 undefined on input line
 889.


Package natbib Warning: Citation `marques17' on page 17 undefined on input line
 889.


Package natbib Warning: Citation `connerney22' on page 17 undefined on input li
ne 889.


Package natbib Warning: Citation `marques17' on page 17 undefined on input line
 889.


Package natbib Warning: Citation `marques17' on page 17 undefined on input line
 889.


Package natbib Warning: Citation `connerney22' on page 17 undefined on input li
ne 889.


Package natbib Warning: There were undefined citations.

[17
pdfTeX warning (ext4): destination with the same identifier (name{figure.A4.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.913 \end{document}
                    
pdfTeX warning (ext4): destination with the same identifier (name{table.A5.1}) 
has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.913 \end{document}
                     <./figs//sketch-vectors-cone.pdf>]
Underfull \vbox (badness 10000) has occurred while \output is active [18
pdfTeX warning (ext4): destination with the same identifier (name{figure.A5.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.913 \end{document}
                     <./figs//io.pdf>]
Underfull \vbox (badness 10000) has occurred while \output is active [19
pdfTeX warning (ext4): destination with the same identifier (name{figure.A6.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.913 \end{document}
                     <./figs//scatter-plots.pdf>] (aux/main.aux

Package natbib Warning: Citation(s) may have changed.
(natbib)                Rerun to get citations correct.

)

LaTeX Font Warning: Size substitutions with differences
(Font)              up to 0.5pt have occurred.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package rerunfilecheck Warning: File `main.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.

 )
(see the transcript file for additional information)
pdfTeX warning (dest): name{Hfootnote.1} has been referenced but does not exist
, replaced by a fixed one

</usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI5.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI7.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.p
fb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi
7.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/c
mr10.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/c
m/cmr5.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts
/cm/cmsy10.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsf
onts/cm/cmsy7.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/a
msfonts/cm/cmtt8.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/publi
c/tex-gyre/qtmr.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public
/newtx/txexs.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/ne
wtx/txmiaX.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/txfo
nts/txsya.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx
/txsys.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/zt
mb.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/ztmr.p
fb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/ztmri.pfb>
Output written on aux/main.pdf (19 pages, 5108675 bytes).
Transcript written on aux/main.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.25 (TeX Live 2023) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2022-11-01> patch level 1
L3 programming layer <2023-02-22> (./mnras.cls
Document Class: mnras 2015/05/22\ v3.0\ LaTeX2e MNRAS document class
MNRAS document style v3.0, released 2015/05/22
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.
sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
 (/usr/local/texlive/2023basic/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/gettitlestring/gettitlestr
ing.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/kvoptions/kvoptions.sty)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty)
) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/atbegshi-ltx.sty)

Package hyperref Warning: Option `pdfpagelabels' is turned off
(hyperref)                because \thepage is undefined.

) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/rerunfilecheck/rerunfilechec
k.sty (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/atveryend-ltx.sty
)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/uniquecounter/uniquecounte
r.sty))) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/natbib/natbib.sty))
 (/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/newtxtext.sty
`newtxtext' v1.71, 2022/02/28 Text macros taking advantage of TeXGyre Termes an
d its extensions (msharpe)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/textcomp.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/carlisle/scalefnt.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kastrup/binhex.tex)
ntx@otftextfalse
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/fontaxes/fontaxes.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.71, 2022/01/16 Math macros based originally on txfonts (msharpe)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifxetex.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/iftex/ifluatex.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/generic/kastrup/binhex.tex)
amsthm NOT loaded
) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fontenc.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1minntx.fd))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/ae.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/base/fontenc.sty))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/aecompl.sty)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/graphics/mathcolor.ltx))
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1ntxtlf.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/l3backend/l3backend-pdftex.d
ef) (aux/main.aux)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/omlntxmi.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(aux/main.out) (aux/main.out)
(/usr/local/texlive/2023basic/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.s
ty
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg
)) (/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/ot1minntx.fd)

LaTeX Font Warning: Font shape `OML/cmm/b/it' in size <10.5> not available
(Font)              size <10.95> substituted on input line 34.

(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/ueur.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/untxsyc.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/t1ntxsups.fd)

LaTeX Font Warning: Font shape `OML/cmm/b/it' in size <5.5> not available
(Font)              size <5> substituted on input line 34.

(/usr/local/texlive/2023basic/texmf-dist/tex/latex/ae/t1aett.fd)
(/usr/local/texlive/2023basic/texmf-dist/tex/latex/newtx/ts1ntxtlf.fd) [1{/usr/
local/texlive/2023basic/texmf-var/fonts/map/pdftex/updmap/pdftex.map}{/usr/loca
l/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ec-tlf.enc}{/usr/local
/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ot1-tlf.enc}{/usr/local
/texlive/2023basic/texmf-dist/fonts/enc/dvips/tex-gyre/q-ts1.enc}]
Underfull \vbox (badness 10000) has occurred while \output is active [2{/usr/lo
cal/texlive/2023basic/texmf-dist/fonts/enc/dvips/newtx/ntx-ec-tlf-pc.enc}]
[3
pdfTeX warning (ext4): destination with the same identifier (name{table.1}) has
 been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.205 \end{equation}
                    ] [4
pdfTeX warning (ext4): destination with the same identifier (name{figure.1}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.230 \end{equation}
                    
pdfTeX warning (ext4): destination with the same identifier (name{figure.2}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.230 \end{equation}
                     <./figs//sketch-geometry.pdf> <./figs//sketch-star-planet-
line.pdf>] [5
pdfTeX warning (ext4): destination with the same identifier (name{figure.3}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.309 
       <./figs//field-lines.pdf>] [6
pdfTeX warning (ext4): destination with the same identifier (name{figure.4}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.357 
       <./figs//quadrature-angles.pdf>] [7
pdfTeX warning (ext4): destination with the same identifier (name{table.2}) has
 been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.432 
      
pdfTeX warning (ext4): destination with the same identifier (name{figure.5}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.432 
       <./figs//quadrature-lc.pdf>]
Underfull \vbox (badness 10000) has occurred while \output is active [8
pdfTeX warning (ext4): destination with the same identifier (name{figure.6}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.457 \begin{equation}
                       <./figs//quadrature-pd.pdf>]
Underfull \vbox (badness 10000) has occurred while \output is active [9
pdfTeX warning (ext4): destination with the same identifier (name{figure.7}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.474 
       <./figs//prob-density-2d.pdf>] [10] [11
pdfTeX warning (ext4): destination with the same identifier (name{figure.8}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.576 A
       n interesting result from these configurations is that they produce e...
 <./figs//scatter-star.pdf>] [12
pdfTeX warning (ext4): destination with the same identifier (name{figure.9}) ha
s been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.625 
       <./figs//planet-hists.pdf>]
Underfull \vbox (badness 10000) has occurred while \output is active [13
pdfTeX warning (ext4): destination with the same identifier (name{figure.10}) h
as been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.641 
       <./figs//c1-c2.pdf>] [14
pdfTeX warning (ext4): destination with the same identifier (name{figure.11}) h
as been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.666 
       <./figs//sketch-c1.pdf>] (aux/main.bbl
Underfull \hbox (badness 1122) in paragraph at lines 202--207
\T1/ntxtlf/m/n/8 ond Work-shop on the LLVM Com-piler In-fras-truc-ture in HPC.
[15]

Package hyperref Warning: Suppressing empty link on input line 321.

) [16
pdfTeX warning (ext4): destination with the same identifier (name{figure.A1.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.811 
       <./figs//sketch-vectors-star.pdf>] [17
pdfTeX warning (ext4): destination with the same identifier (name{figure.A2.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.906 \end{figure*}
                   
pdfTeX warning (ext4): destination with the same identifier (name{figure.A4.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.906 \end{figure*}
                   
pdfTeX warning (ext4): destination with the same identifier (name{table.A5.1}) 
has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.906 \end{figure*}
                    <./figs//sketch-vectors-planet.pdf> <./figs//sketch-vectors
-cone.pdf>] [18
pdfTeX warning (ext4): destination with the same identifier (name{figure.A5.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.913 \end{document}
                     <./figs//io.pdf>]
Underfull \vbox (badness 10000) has occurred while \output is active [19
pdfTeX warning (ext4): destination with the same identifier (name{figure.A6.1})
 has been already used, duplicate ignored
<argument> ...shipout:D \box_use:N \l_shipout_box 
                                                  \__shipout_drop_firstpage_...
l.913 \end{document}
                     <./figs//scatter-plots.pdf>] (aux/main.aux)

LaTeX Font Warning: Size substitutions with differences
(Font)              up to 0.5pt have occurred.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information)
pdfTeX warning (dest): name{Hfootnote.1} has been referenced but does not exist
, replaced by a fixed one

</usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI5.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/NewTXMI7.pfb><
/usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.p
fb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi
7.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/cm/c
mr10.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts/c
m/cmr5.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsfonts
/cm/cmsy10.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/amsf
onts/cm/cmsy7.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/a
msfonts/cm/cmtt8.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/publi
c/tex-gyre/qtmr.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public
/newtx/txexs.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/ne
wtx/txmiaX.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/txfo
nts/txsya.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx
/txsys.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/zt
mb.pfb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/ztmr.p
fb></usr/local/texlive/2023basic/texmf-dist/fonts/type1/public/newtx/ztmri.pfb>
Output written on aux/main.pdf (19 pages, 5121292 bytes).
Transcript written on aux/main.log.

